Induction Models on \mathbb{N}

Mathematical induction is a fundamental tool in computer science and mathematics. Henkin initiated the study of formalization of mathematical induction restricted to the setting when the base case B is set to singleton set containing 0 and a unary generating function S. The usage of mathematical induction often involves wider set of base cases and k-ary generating functions with different structural restrictions. While subsequent studies have shown several Induction Models to be equivalent, there does not exist precise logical characterization of reduction and equivalence among different Induction Models. In this paper, we generalize the definition of Induction Model and demonstrate existence and construction of S for given B and vice versa. We then provide a formal characterization of the reduction among different Induction Models that can allow proofs in one Induction Models to be expressed as proofs in another Induction Models. The notion of reduction allows us to capture equivalence among Induction Models.

==> results.tex <==
\section{Main Technical Results}
\label{sect:main_results}

The following are the main theorems of this paper. Details can be found in sections \ref{sect: characterisation} and \ref{sect:reduction_equivalence}.



%\begin{description}
	%\item[Formalization of $\mathbb{N}$-Induction Models] : We formally define $\mathbb{N}$-Induction Model via the necessary and sufficient properties for $B$ and $S$ to constitute $\langle B,S \rangle$ to be an $\mathbb{N}$-Induction Model. We also show that $Cl(\langle B, S \rangle) = \mathbb{N}$ if and only if $\langle B, S \rangle$ is an $\mathbb{N}$-Induction Model. ({\bfseries Definition \ref{def: N_induction_model} and Theorem \ref{lemma: mi_definitions_are_equivalent}})
	
	%\item[Finding $B$ and $S$:]
	%We prove that for every non-self-loop function $S: \mathbb{N}^k \rightarrow \mathbb{Z}$, there exists a $B \subset \mathbb{N}$ such that $\langle B, S \rangle$ is an $\mathbb{N}$-Induction Model. So this is true for $S$ with additive and multiplicative structures. We prove that for every non-empty $B \subset \mathbb{N}$ and $k$, there exists a $k$-ary non-self-loop function $S: \mathbb{N}^k \rightarrow \mathbb{Z}$, such that $\langle B, S \rangle$ is an $\mathbb{N}$-Induction Model. We prove the same for functions with additive structure. We also show that if $S$ is unary, $\langle B,S \rangle$ is an $\mathbb{N}$-I.M. iff $B$ contains 1 or it is an infinite set. For functions with multiplicative structure, we prove this result for $B$ containing at least 2 elements. {\bfseries (Theorem \ref{theorem: summary_finding_B_and_S})}
	
	%\begin{description}
	 %   \item[Existence of S for every B:] We prove that for every non-empty $B \subset \mathbb{N}$ and $k$, there exists a $k$-ary non-self-loop function $S: \mathbb{N}^k \rightarrow \mathbb{Z}$, such that $\langle B, S \rangle$ is an $\mathbb{N}$-Induction Model. We extend the proof that there also exists a $S$ with additive structure and another $S$ with product structure such that $\langle B, S \rangle$ is an $\mathbb{N}$-Induction Model. ({\bfseries Lemma \ref{lemma: every_b_there_is_s_extended_version}, Lemma \ref{lemma: additive_S_every_B_there_is_S_extended_version}, and Lemma \ref{multiplicative_every_B_there_is_S_any_two_extended_version}})
	    
	  %\item[Existence of $B$ for every $S$]:  Extending the proof, we also show that there exists $B$ for every $S$ with additive or product structure as well such that $\langle B, S \rangle$ is an $\mathbb{N}$-Induction Model. ({\bfseries Lemma \ref{lemma: every_s_there_is_b}, Lemma \ref{lemma: additive_S_every_S_there_is_B}, and Lemma \ref{multiplicative_every_S_there_is_B}})
	%\end{description}
	  
	%\item[Reduction and Equivalence of Induction Models]: We give a definition for reduction and equivalence of Induction Models. We present a criterion to determine if one Induction Model can be reduced to another Induction Model. Moreover, we also give a criterion to check when two Induction Models are equivalent. In the end, we prove that every $\mathbb{N}$-Induction Models can be reduced to $\langle B_0,S_0 \rangle$. {\bfseries (Theorem \ref{theorem: equivalent_condition_reduction})}
%\end{description}
